Exploring the Loss Landscape in Neural Architecture Search

Neural architecture search (NAS) has seen a steep rise in interest over the last few years. Many algorithms for NAS consist of searching through a space of architectures by iteratively choosing an architecture, evaluating its performance by training it, and using all prior evaluations to come up with the next choice. The evaluation step is noisy - the final accuracy varies based on the random initialization of the weights. Prior work has focused on devising new search algorithms to handle this noise, rather than quantifying or understanding the level of noise in architecture evaluations. In this work, we show that (1) the simplest hill-climbing algorithm is a powerful baseline for NAS, and (2), when the noise in popular NAS benchmark datasets is reduced to a minimum, hill-climbing to outperforms many popular state-of-the-art algorithms. We further back up this observation by showing that the number of local minima is substantially reduced as the noise decreases, and by giving a theoretical characterization of the performance of local search in NAS. Based on our findings, for NAS research we suggest (1) using local search as a baseline, and (2) denoising the training pipeline when possible.

==> impact.tex <==

Our work seeks to improve the understanding of neural architecture search
by analyzing the differences between benchmark vs.\ large-scale
search spaces, characterizing the performance of local search,
and helping to lay the groundwork for future theoretical results.
While this does not have an immediate societal impact the same way
that a GAN for deep fakes or a deep learning optimizer for $\text{CO}_2$ emissions
would, our work, and more broadly the field of NAS, will be the algorithms
powering and refining the deep learning applications with direct societal
implications.

Since our work only indirectly affects society,
we have less control over its net implications.
However, we see two benefits to the AI community that will foster
a positive impact. First, we help to lay the groundwork for future theoretical
results which can improve our understanding of the workings of different algorithms.
Second, we present an easily implementable NAS algorithm which gives strong performance
under some settings, and we advocate for simpler NAS algorithms in the future.
Not only will this exhibit better baselining of NAS algorithms, but it also helps to
democratize neural architecture search. Easily implementable and understandable NAS
algorithms will lead to more widespread use.
Because of the recent push for explicitly reasoning about the impact of
research in AI~\cite{hecht2018time}, we are hopeful that downstream deep learning
applications will be used to benefit society.


